On the Inefficiency of the Merit Order in Forward Electricity Markets with Uncertain Supply

This paper provides insight on the economic inefficiency of the classical merit-order dispatch in electricity markets with uncertain supply. For this, we consider a power system whose operation is driven by a two-stage electricity market, with a forward and a real-time market. We analyze two different clearing mechanisms: a conventional one, whereby the forward and the balancing markets are independently cleared following a merit order, and a stochastic one, whereby both market stages are co-optimized with a view to minimizing the expected aggregate system operating cost. We first derive analytical formulae to determine the dispatch rule prompted by the co-optimized two-stage market for a stylized power system with flexible, inflexible and stochastic power generation and infinite transmission capacity. This exercise sheds light on the conditions for the stochastic market-clearing mechanism to break the merit order. We then introduce and characterize two enhanced variants of the conventional two-stage market that result in either price-consistent or cost-efficient merit-order dispatch solutions, respectively. The first of these variants corresponds to a conventional two-stage market that allows for virtual bidding, while the second requires that the stochastic power production be centrally dispatched. Finally, we discuss the practical implications of our analytical results and illustrate our conclusions through examples.

==> table4_1.tex <==
"fore"	"inef"	"vb"
0.1	0.285421387081245	0.179514379287394
0.2	0.51397662322221	0.325979656365269
0.3	0.772273627110087	0.478589645317395
0.4	1.06785958667987	0.650356434557127
0.5	1.4154825404913	0.839873045072403
0.6	1.84281707052757	1.04972196672142
0.7	2.41027494357321	1.2737424167848
0.8	3.26068175484681	1.44830454173506
0.9	4.1644798333315	0.997321674005698


==> table4_24.tex <==
"fore"	"inef"	"vb"
0.1	0.384045645233469	0.25407434020356
0.2	0.640838802189976	0.411170945225746
0.3	0.925345140851143	0.580369157550222
0.4	1.25183775681538	0.765513220705132
0.5	1.64119601436837	0.971622817571267
0.6	2.12767882736821	1.2004011927907
0.7	2.78727606688364	1.44033560431244
0.8	3.7871017958194	1.58881036004669
0.9	4.59378010629513	1.00224765524417


==> table4_48.tex <==
"fore"	"inef"	"vb"
0.1	0.493690234312308	0.346408782256722
0.2	0.784556291484947	0.513095963624915
0.3	1.10222285054059	0.698621474466275
0.4	1.46573686616195	0.901365889926672
0.5	1.90302821254788	1.12511885398404
0.6	2.45786073390841	1.37287263710356
0.7	3.2273186021195	1.62413851950164
0.8	4.38682999395099	1.71666453509634
0.9	5.02418046650906	1.0073165391577

